PeFLL: Personalized Federated Learning by Learning to Learn

We present PeFLL, a new personalized federated learning algorithm that improves over the state-of-the-art in three aspects: 1) it produces more accurate models, especially in the low-data regime, and not only for clients present during its training phase, but also for any that may emerge in the future; 2) it reduces the amount of on-client computation and client-server communication by providing future clients with ready-to-use personalized models that require no additional finetuning or optimization; 3) it comes with theoretical guarantees that establish generalization from the observed clients to future ones. At the core of PeFLL lies a learning-to-learn approach that jointly trains an embedding network and a hypernetwork. The embedding network is used to represent clients in a latent descriptor space in a way that reflects their similarity to each other. The hypernetwork takes as input such descriptors and outputs the parameters of fully personalized client models. In combination, both networks constitute a learning algorithm that achieves state-of-the-art performance in several personalized federated learning benchmarks.

==> ablation_studies/embedding_net_architecture_ablation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{|c|ccc|ccc|}
        \hline
        &\multicolumn{3}{c|}{CIFAR10} & \multicolumn{3}{c|}{CIFAR100} \\
        \hline
        \#Clients & 100 & 500 & 1000 & 100 & 500 & 1000 \\
        \hline
        MLP & $88.5 \pm 1.2$ & $87.8 \pm 1.1$ & $87.5 \pm 2.1$ & $59.1 \pm 0.2$ & $53.4 \pm 0.4$ & $51.2 \pm 0.5$ \\
        CNN & $88.9 \pm 0.7$ & $88.9 \pm 0.3$ & $88.4 \pm 0.4$ & $59.4 \pm 0.2$ & $54.4 \pm 0.3$ & $53.2 \pm 0.3$ \\
        \hline
    \end{tabular}
    \caption{Test accuracy on CIFAR10 and CIFAR100 using different embedding network architectures. MLP is a single hidden layer fully connected network and CNN is a LeNet-style ConvNet.}
    \label{tab:my_label}
\end{table}

==> ablation_studies/hnet_size_ablation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{|c|ccc|ccc|}
        \hline
        &\multicolumn{3}{c|}{CIFAR10} & \multicolumn{3}{c|}{CIFAR100} \\
        \hline
        \#Clients & 100 & 500 & 1000 & 100 & 500 & 1000 \\
        \hline
        S & $88.7 \pm 0.3$ & $88.2 \pm 0.4$ & $87.7 \pm 0.4$ & $57.9 \pm 0.3$ & $51.9 \pm 0.6$ & $47.4 \pm 1.4$ \\
        M & $88.9 \pm 0.7$ & $88.9 \pm 0.3$ & $88.1 \pm 0.3$ & $59.4 \pm 0.2$ & $53.1 \pm 0.4$ & $50.8 \pm 0.5$ \\
        L & $88.7 \pm 0.8$ & $88.8 \pm 0.3$ & $88.2 \pm 0.6$ & $59.8 \pm 0.1$ & $53.8 \pm 0.2$ & $52.6 \pm 1.0$ \\
        \hline
    \end{tabular}
    \caption{Test accuracy on CIFAR10 and CIFAR100 using different sizes of hypernetworks, small (S), medium (M) and large (L).}
    \label{tab:hnet_size}
\end{table}

==> ablation_studies/regularization_ablation_cifar10_test_clients.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
        & $0$ & $5e-05$ & $5e-03$ & $5e-01$ \\
        \hline
        0 &$87.4 \pm 1.1$ & $89.0 \pm 0.7$ & $87.7 \pm 0.8$ & $82.5 \pm 1.5$ \\
        $1e-05$ & $87.4 \pm 1.0$ & $88.7 \pm 0.6$ & $87.6 \pm 0.8$ & $83.8 \pm 1.1$ \\
        $1e-03$ & $88.4 \pm 0.6$ & $88.8 \pm 0.3$ & $87.5 \pm 0.5$ & $86.2 \pm 0.4$\\
        \hline
    \end{tabular}
    \caption{Test accuracy on train clients, along top is regularization of the client network, on the left is regularization of the hypernetwork and embedding network}
    \label{tab:my_label}
\end{table}

==> ablation_studies/regularization_ablation_cifar10_train_clients.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
        & $0$ & $5e-05$ & $5e-03$ & $5e-01$ \\
        \hline
        0 &$87.4 \pm 1.1$ & $89.0 \pm 0.7$ & $87.8 \pm 0.8$ & $82.5 \pm 1.5$ \\
        $1e-05$ & $87.4 \pm 1.0$ & $88.7 \pm 0.6$ & $87.6 \pm 0.8$ & $83.8 \pm 1.1$ \\
        $1e-03$ & $88.4 \pm 0.6$ & $88.8 \pm 0.3$ & $87.5 \pm 0.5$ & $86.2 \pm 0.4$\\
        \hline
    \end{tabular}
    \caption{Test accuracy on train clients, along top is regularization of the client network, on the left is regularization of the hypernetwork and embedding network}
    \label{tab:my_label}
\end{table}
